Julia for Biologists

Increasing emphasis on data and quantitative methods in the biomedical sciences is making biological research more computational. Collecting, curating, processing, and analysing large genomic and imaging data sets poses major computational challenges, as does simulating larger and more realistic models in systems biology. Here we discuss how a relative newcomer among computer programming languages -- Julia -- is poised to meet the current and emerging demands in the computational biosciences, and beyond. Speed, flexibility, a thriving package ecosystem, and readability are major factors that make high-performance computing and data analysis available to an unprecedented degree to "gifted amateurs". We highlight how Julia's design is already enabling new ways of analysing biological data and systems, and we provide a, necessarily incomplete, list of resources that can facilitate the transition into the Julian way of computing.

==> old figures and code/old_abstraction_intro.tex <==
Compared to other programming languages such as R and Python or C and C++, Julia allows an exceptionally high level of abstraction. 
We can use the analogy to the "pipettor" to develop some intuition for what we mean by abstraction, and why it is a useful feature for scientific programming. The pipettor is a standard piece of lab equipment made with slightly different designs by many different manufacturers that nevertheless all perform the same task: ``they have the same abstract interface". It thus takes minimum effort to adapt to a new pipettor and the scientist can go on with their lab work without having to care about the details of their tool (the pipettor).
\par
Abstraction achieves the same for software and an abstract interface allows us to adapt and reuse code with minimal adaptation or rewriting of code. Julia's abstraction capabilities allow us to generate and exploit the advantages of different software implementations with different internal characteristics without an overall performance penalty. Some concrete examples below will make this clearer.
%In this analogy we can think of Julia as the person who can pick up any particular pipettor and seamlessly customize their grip, pressure, and other movements in order to use the new pipettor with optimal efficiency. In contrast, most other languages are either limited to a single kind of pipettor or are so unoptimized that they have to perform a lengthy (re)calibration before every single operation. The combination of abstraction (all pipettors have a common "interface") coupled with specialization (Julia customizes specific muscle movements to the demands of that specific pipettor) allows Julia to exploit many implementations with different internal characteristics without a performance penalty. This in turn leads to flexibility: biologists can implement models at an appropriate degree of detail, without compromising on performance, and with the code being reusable in other contexts.
%In order to develop an intuition for abstraction, we want to draw an analogy to a more established tool of the biologist, the "pipettor". The pipettor is a standard piece of lab equipment made with slightly different designs by many different manufacturers that nevertheless all perform the same task (they have the same abstract interface). In this analogy we can think of Julia as the person who can pick up any particular pipettor and seamlessly customize their grip, pressure, and other movements in order to use the new pipettor with optimal efficiency. In contrast, most other languages are either limited to a single kind of pipettor or are so unoptimized that they have to perform a lengthy (re)calibration before every single operation. The combination of abstraction (all pipettors have a common "interface") coupled with specialization (Julia customizes specific muscle movements to the demands of that specific pipettor) allows Julia to exploit many implementations with different internal characteristics without a performance penalty. This in turn leads to flexibility: biologists can implement models at an appropriate degree of detail, without compromising on performance, and with the code being reusable in other contexts.
\par 
Compared to, for example, physics, the biological sciences have  a high level of heterogeneity in the available data
\cite{Alyass2015, GomezCabrero2014, Nagaraj2018}. A language design that promotes abstraction, enabling easy and elegant reuse of existing code, can therefore make biologists' work more straightforward. % It enables the biologist to design, realise and implement biological studies much faster.
Defining intuitive representations of biological problems is important as it reduces the chance of misinterpretation and mistakes.
In this way Julia's abstract language design enables scientists to improve the accuracy and correctness of biological studies. Appropriately complex descriptions are sometimes avoided in other languages due to incompatibility issues with existing code. Julia's generic code design enables elegant solutions to reuse code for new, user specific problems.
\par 
Julia's support for abstraction also enables and encourages collaborative software development. It provides easy access to robust and high performance code through Julia's rapidly expanding package ecosystem (Figure \ref{fig:packages} and Table \ref{tab:packages}). This has two advantages. First, experts across many fields have curated, optimised and benchmarked these packages. This means users can build their projects on top of existing packages, knowing that they are taking advantage of robust and highly optimised code. Second, because of the low barrier between user and developer, every new user quickly becomes capable of reviewing, improving and contributing to the  Julia language and its package ecosystem. 


==> old figures and code/old_img_sec.tex <==

Image processing is fundamental to disciplines such as cell biology and neuroscience. Images are typically represented as arrays, and they exhibit tremendous diversity: a single picture may have two spatial dimensions and possibly a ``color channel'' for red, green, and blue components; alternatively they may have three spatial dimensions and/or a time dimension, or be hyperspectral\cite{??}. Scientific images may be acquired with 8-bit, 16-bit, or even 12-bit cameras, and detecting which pixels are saturated (i.e., those for which intensity exceeded the limits of acquisition, jeopardizing quantitative analysis) cannot always be determined just from the bit-level representation. Images can also be very large, sometimes reaching multiple terabytes (e.g., a three-dimensional calcium imaging time series as acquired by light sheet fluorescence microscopy\cite{Holekamp2008} or electron microscopy connectomics\cite{??}).

Software to analyze images needs to handle this diversity in representation without compromising performance. Moreover, biological meaning often cannot be extracted without some form of ``data cleaning'' or change in representation. For example, imagine creating an image viewer suitable for visualizing a time series of two-dimensional images. An inflexible viewer would require a very specific data format, for example a literal 3-dimensional array \texttt{img[x, y, t]} of \texttt{UInt8} numbers to represent grayscale intensity at each position and time, and it would simply render these intensities to the screen. But now imagine that you want to manipulate the contrast during visualization to enhance features of interest. You are now faced with a choice: do you implement support for this operation in the viewer, or do you require that the user create a new image, \texttt{img2[x, y, t]}, in which the contrast has been manipulated in the array? If \texttt{img} is a large time series of tens of gigabytes, generating an altered-contrast version of the movie would require writing a second disk file of the raw data with significant cost in time and effort. Thus, one is incentivized to add a feature directly to the viewer to support altered contrast.

But now suppose that you need to support more operations: examples might include any combination of background subtraction, real-time motion correction, feature recognition and highlighting, and visualization paired with image quantification. These high-level operations might require a large collection of lower-level tools, like the ability to crop the image or blank out a time stamp embedded in the image prior to image alignment, spatiotemporal filtering, etc. What if, to support interactive visualization, you'd like to perform these operations in real-time without requiring the user to generate a nearly-endless series of altered versions of the movie on disk? Which of these operations need to be performed just at rendering time, and which need to be performed prior to a previous manipulation? Should cropping be performed before alignment or after? The feature set and user-interface complexity of the combined viewer/analyzer may grow rapidly as one tries to create a tool that covers such uses.

While writing such a viewer is feasible in Julia and many other languages, Julia provides a practical alternative that is easy, performant, and infinitely flexible.  The basic concept is support for \emph{lazy operations}, declaring the computation you want to perform but deferring its execution until the last possible moment. For example, you can manipulate the contrast by rendering \texttt{f(img[x, y, t])}, where \texttt{f} is some function that modifies the intensity of a pixel; similarly, you can spatially warp the image by rendering \texttt{img[gx(x, y, t), gy(x, y, t), t]} for coordinate-transformations \texttt{gx} and \texttt{gy}. When you directly call \texttt{f(img[x, y, t])} to manipulate the contrast, this \emph{eager operation} gets run immediately; but Julia also has the MappedArrays.jl package\cite{MappedArrays}, with which you can declare \texttt{img2 = mappedarray(f, img)}. \emph{Creating} \texttt{img2} is instantaneous and takes virtually no memory regardless of the size of \texttt{img}, because the computation is performed only when accessing \texttt{img2[x, y, t]}, which returns \texttt{f(img[x, y, t])} by referencing the original \texttt{f} and \texttt{img}. This allows you to manipulate contrast in a multi-terabyte memory-mapped image on a standard laptop. Such operations are possible in other languages too, but often at the cost of performance-killing overhead; in Julia, there is no more overhead than that of computing \texttt{f(value)} itself.  Moreover, \texttt{img2} can be passed to a ``dumb'' image viewer with no understanding of how to manipulate contrast. Similarly, Julia's ImageTransformations.jl package\cite{ImageTransformations} lets you declare \texttt{img3 = warpedview(img2, g)}
to apply a coordinate transformation \texttt{g} to each pixel before visualization, again using nothing but lazy operations. 
Because Julia has a standard \texttt{AbstractArray} interface\cite{AbstractArrays, MultidimIteration}, such manipulations may be chained together, creating novel array types like a new structure made from individual transformations.  This allows you to build an extensive ``data cleaning'' pipeline customized to the needs of each data set, and pass the resulting image to analysis or visualization code that can be written to be independent of all these transformations.

For supporting such operations, one of Julia's key characteristics is that of \emph{compile-time function specialization}: when you call \texttt{viewimage(A)} on some array \texttt{A}, Julia will compile a dedicated version of \texttt{viewimage} for any special features (encoded by the type system) of \texttt{A}. One version might be compiled to handle ``plain" 3d arrays of \texttt{UInt8} pixels, but a completely independent version would be compiled to handle a ``lazy array" that has been spatio-temporally altered. Because Julia's compiler optimizes aggressively, there is typically no overhead to this flexibility: the compiler generates a series of computations that run as efficiently as if you had directly implemented the feature in the visualizer itself. This process is illustrated in Box~\ref{box:Lazy}, an example that combines contrast adjustment, spatial manipulation, and multiple-image overlay entirely lazily and yet which can be viewed at 30fps on ordinary laptop hardware.

% \begin{BOX}[H]
%     \centering
%     \fbox{\parbox{\textwidth}{
%     Using a trivial visualizer to play a ``movie'' with ``on the fly'' manipulations:
%     \begin{itemize}
%         \item Convert digital numbers to photons
%         \item Square-root transform to yield Gaussian noise
%         \item Continuously spin the image (a simple spatial transformation)
%         \item Overlay with other images (to mimic a test of image registration)
%     \end{itemize}
    
%     \lstinputlisting[language=Julia]{code_example_images.jl} % This code is not running for me.
%     \caption{Julia's abstraction enables efficient lazy operations on data sets far larger than the memory resources of the machine.  Of note, in this pipeline the only arrays that actually store raw data are the imagined input \texttt{img}, a 2d+time grayscale image, and \texttt{imgref}, a 2d reference image; all other arrays are lazy, yet can be used with no extra overhead.\label{box:Lazy}}
%     }}
% \end{BOX}

These features enable new analyses and experiments. For example, Julia has been adopted by labs processing large images acquired by light sheet microscopy in mice\cite{Lee2019} and fish\cite{??}. Julia also enabled a real-time two-photon pipeline to perform calcium imaging in intact neural tissue and then select and phototag specific cells that exhibited specific response properties\cite{Lee2019}.
The tagged cells were then harvested for sequencing to determine their patterns of gene expression, resulting in new discoveries about the receptor genes underlying detection of socially-relevant odors.

% As a further example of the power of Julia's abstractions, consider the task of writing an algorithm to support arrays of arbitrary dimension. In many languages, supporting multiple dimensions generically is exceptionally painful, slow, and/or very limited. In contrast, Julia makes such support straightforward without performance penalty. For example, writing a "boxcar" filter---in which one averages over boxes centered at each location---has an inner loop such as:

% \begin{verbatim}
%     # Given an `n`-dimensional array `input`, compute the average value in a
%     # multidimensional box of half-width `W[1], ..., W[n]` around the
%     # location `I[1], ..., I[n]`:
%     s = n = 0
%     for J in max(Ifirst, I-W):min(Ilast, I+W)   # this spans I-W : I+W, but truncates at the edges
%         s += input[J]                           # accumulator for value
%         n += 1                                  # accumulator for number of locations visited
%     end
%     output[I] = s/n                             # average value
% \end{verbatim}
% Despite its simplicity, this code is remarkably robust: it gracefully handles cases in which one dimension of \texttt{input} might be smaller than the corresponding dimension of \texttt{2W+1}, and at array edges it naturally uses just the data that are available.

% The ability to perform efficient computations with multidimensional indices opens the door to a straightforward implementations of a wide variety of algorithms. A more complex example is shown in Box~??, an algorithm designed by Maurer, Qi, and Raghavan to compute the distance to the closest `true`-valued array element from any other point in the array (this is implemented as \texttt{bwdist} in Matlab and \texttt{morphology.distance\_transform\_edt} in scikit-image). This algorithm involves multidimensional loops (see the \texttt{...} in the pseudocode), with computation occurring along a chosen dimension `d`, and recursion across dimensions (line 11).  The innermost call for \texttt{d=1} (lines 3--7) is a performance hotspot. While writing such an algorithm in full generality might be daunting in most languages, one sees that the Julia implementation is even shorter than the pseudocode. Despite being an almost "brainless" translation of the pseudocode, it runs 20\% \emph{faster} on a thread-by-thread basis than Matlab's \texttt{bwdist} (which, from the absence of m-file code, appears to be written in C).

